Storytelling in human--centric software engineering research

BACKGROUND: Software engineering is a human activity. People naturally make sense of their activities and experience through storytelling. But storytelling does not appear to have been properly studied by software engineering research. AIM: We explore the question: what contribution can storytelling make to human--centric software engineering research? METHOD: We define concepts, identify types of story and their purposes, outcomes and effects, briefly review prior literature, identify several contributions and propose next steps. RESULTS: Storytelling can, amongst other contributions, contribute to data collection, data analyses, ways of knowing, research outputs, interventions in practice, and advocacy, and can integrate with evidence and arguments. Like all methods, storytelling brings risks. These risks can be managed. CONCLUSION: Storytelling provides a potential counter--balance to abstraction, and an approach to retain and honour human meaning in software engineering.

==> sections/X_3_rationale_for_story_in_SE.tex <==
\section{Rationale for a vision}

\subsection*{Notes}

\begin{enumerate}
    \item SE is multidisciplinary
    \item Within SE research, there is the emergence of human--centric software engineering and behavioural software engineering. These place people at the centre of software engineering.
    \begin{itemize}
        \item Meaning, and abstraction
        \item Beliefs -- Devanbu eg al. 
        \item Values
        \item Experiences
        \item Motivation
        \item Happiness
    \end{itemize}
    \item There are fundamental challenges to software engineering research
    \begin{itemize}
        \item Context \& postmodernism
        \item Quote EBSE and discuss
        \item What constitutes evidence
        \item What constitutes acceptable knowledge
        \begin{itemize}
            \item For practice cf. Rainer's persuading paper
            \item For research
            \item Methodical and amethodical
        \end{itemize}
        \item What is acceptable methodology
    \end{itemize}
    \item There is a greater awareness of the impact of software engineering and of the value system within which software engineering takes place. These can't be addressed within existing ways of knowing and accepted types of knowledge.
    \item Counter--balance to `big data' and AI/ML
    \item Counter--balance to abstraction cf. quote McGee Paw
\end{enumerate}

\subsection{Story and storytelling in research}

Stories are recognised as a legitimate focus of study in other scientific disciplines, e.g., energy and climate change research \cite{moezzi2017using}, law \cite{anderson2005analysis, twining1994rethinking}, organisational research \cite{weick1995sensemaking}, and behavioural medicine \cite{shaffer2018usefulness}. And whilst story and storytelling is recognised in a variety of disciplines related to software engineering (e.g., information systems \cite{Schwabe2019specialissue}, human--computer interaction \cite{blythe2017research}, computer supported cooperative work \cite{orr1986narratives}, information visualisation \cite{gershon2001storytelling}, multimedia systems \cite{lugmayr2017serious} and computer science education \cite{kelleher2007using, naul2020story}), software engineering \textit{research} has tended to direct attention only at one particular type of \textit{story}, i.e., the user story. 

In behavioural medicine, Shaffer et al. \cite{shaffer2018usefulness} cite prior work to assert several benefits with narrative--as--story. But Shaffer et al. \cite{shaffer2018usefulness} also write that, ``\dots interventions with narratives appear to escape the scrutiny that interventions with statistical evidence receive from people who disagree with the message. This has important implications for health behavior change interventions [and, for the current paper, there are important implications for interventions in software engineering practice], where the goal is often to change attitudes towards an unhealthy or harmful health behavior [or, for the current paper, the goal of improving a suboptimal or counterproductive software practice].'' (\cite{shaffer2018usefulness}, p. 431).We briefly review Shaffer et al.'s work \cite{shaffer2018usefulness, shaffer2013all} later in this paper.

% that such narrative is more engaging than didactic presentations; that there is more engagement from the reader with a narrative message than with a statistical message; that narratives are perceived to be more relevant (the relevance of software engineering research is a long--running issue, e.g., \cite{lo2015practitioners}); that narrative is more effective at communicating information; and that narrative is read more quickly and information is more accurately recalled. (We discuss the effects of story later in this paper.)

There is some attention in software engineering research directed at narrative analysis and synthesis (e.g., \cite{cruzes2015case}) however that work uses the term \textit{narrative} in the sense of the qualitative inquiry into and with texts rather than as \textit{story}. We find several papers that explicitly recognise story and storytelling in software engineering research: Ahonen and Sihvonen's \cite{ahonen2005things} story of software process improvement; Lenberg et al.'s unpublished manuscript \cite{lenberg2017behavioral} on guidelines for qualitative studies of behavioural software engineering; and a several papers (e.g., \cite{lutters2007revealing,sim2011getting}) that study war stories using storytelling as a method of data collection. We consider these publications later in this paper.
% (though there are others, e.g., using storytelling to teach programming \cite{kelleher2007using}).

==> sections/X_5_realising_the-vision.tex <==
\section{Steps toward realising the vision}

\subsection*{Notes}

\begin{enumerate}
    \item Focus here on research, but at least some applies to practice
    \begin{itemize}
        \item Steps for research
        \item Steps for practice
    \end{itemize}
    \item Develop frameworks or models cf. AXE
    \item Developing new skills
    \item Reading groups
    \item Writing groups cf. Faber Academy
    \item Storytelling platforms \& resources
    \begin{itemize}
        \item Network
        \item StoryCorps
        \item Agile Corps
        \item Story Collider
    \end{itemize}
    \item Dissemination of \textit{argued stories} and \textit{evidence--based storytelling}
    \begin{itemize}
        \item Conference workshop/s
        \item Sections in journals 
    \end{itemize}
    \item Change to metrics of impact
    \item Standards for acceptable empirical research in SE
    \item Multidisciplinary collaboration
    \item Supplementary materials (papers as code, papers as story)
    \begin{itemize}
        \item cf. PROMISE
        \item papers with code
    \end{itemize}
    \item Methodology
    \begin{enumerate}
        \item War story interview
        \item Story Stem Technique
        \item Protocol/s for handling stories
        \begin{enumerate}
            \item Argument schemes
            \item Legal protocols
        \end{enumerate}
        \item Integrating story with other kinds of knowing
    \end{enumerate}
\end{enumerate}
